Zero-Shot Semantic Segmentation via Spatial and Multi-Scale Aware Visual Class Embedding

Fully supervised semantic segmentation technologies bring a paradigm shift in scene understanding. However, the burden of expensive labeling cost remains as a challenge. To solve the cost problem, recent studies proposed language model based zero-shot semantic segmentation (L-ZSSS) approaches. In this paper, we address L-ZSSS has a limitation in generalization which is a virtue of zero-shot learning. Tackling the limitation, we propose a language-model-free zero-shot semantic segmentation framework, Spatial and Multi-scale aware Visual Class Embedding Network (SM-VCENet). Furthermore, leveraging vision-oriented class embedding SM-VCENet enriches visual information of the class embedding by multi-scale attention and spatial attention. We also propose a novel benchmark (PASCAL2COCO) for zero-shot semantic segmentation, which provides generalization evaluation by domain adaptation and contains visually challenging samples. In experiments, our SM-VCENet outperforms zero-shot semantic segmentation state-of-the-art by a relative margin in PASCAL-5i benchmark and shows generalization-robustness in PASCAL2COCO benchmark.

==> body/3/3.td.tex <==
\section{Task Description}
The goal of ZSSS is to perform segmentation on a novel class that is unseen during the training phase. 
Here, we define the set of classes for training $C_{train}$ and test $C_{test}$. 
From the global classes $C_{global} = \{ c_1, c_2, ..., c_{\infty} \}$ that includes every class in the real-world, there are $n$ training classes $C_{train}=\{ c_1, c_2, ..., c_n \}$ and $m$ target classes for test $C_{test}=\{ c_{n+1}, c_{n+2}, ..., c_{n+m} \}$.
Note that there is no intersecting class between the training classes and the test classes $C_{test} \cap C_{train} = \emptyset$. 

\textbf{ZSSS using word vector.} 
Recent zero-shot semantic segmentation methods~\cite{zsvm, spnet} utilizes word vectors for side information to generate class embedding.
In the ZSSS setting using the word vector, the test set $S^{test}_{word}$ contains tuples of query image and the corresponding word vector. 
The training set $S^{train}_{word}$ consists of query image, label and corresponding word vector.  
Thus, the two sets $S^{train}_{word}$, $S^{test}_{word}$ are defined as follows: 
\[
S^{train}_{word} = \{(I_{i}^{train},L_{i}^{train}, W^{train}_i)\}_{i=1}^{N^{train}}
\]
\[
S^{test}_{word} = \{(I_{j}^{test}, W_j^{test})\}_{j=1}^{N^{test}}
\]
where $N^{train}$ and $N^{test}$ are the number of train and test samples, $I \in \mathbb{R}^{C \times H \times W}$ is an image when $C, H, W$ are the image RGB channels, height and width, $L^s_i \in \{0, 1\}^{H \times W}$ is the label and $W^s_i$ is the word vector of the class of the image $I^s_i$ for $s \in \{ train, test \}$. 

\textbf{ZSSS via Visual Class Embedding} 
In our proposed ZSSS via VCE setting, the training set $S^{train}_{VCE}$ and the test set $S^{test}_{VCE}$ exclude the word vector $W$ as we generate the class embedding from the query image with ImageNet pretrained knowledge.
The train set $S^{train}_{VCE}$ and the test set $S^{test}_{VCE}$ for our ZSSS via VCE setting are defined as follows:
\[
S^{train}_{VCE} = \{(I_{i}^{train},L_{i}^{train})\}_{i=1}^{N_{train}}
\]
\[
S^{test}_{VCE} = \{(I_{j}^{test})\}_{j=1}^{N_{test}}
\]
Given such datasets, our task is to segment an image $I$ into a mask $M \in \{0, 1\}^{H \times W}$, meaning if a pixel belongs to the target class.


==> body/5/0.section_description.tex <==
In this section, we show that domain shift causes changes in visual representations (Section~\ref{domainshift}) and demonstrate three following ZSSS experiments on the unified PASCAL2COCO benchmark.
First in Section~\ref{pascal5i}, we train models on PASCAL-$5^i$ training set and evaluate on PASCAL-$5^i$ test set to compare performances on the train domain. 
Second in Section~\ref{coco20i}, we evaluate the models on COCO-$20^i$ test set to see generalization ability and performances on visually challenging cases.
Lastly in Section~\ref{ablation}, we conducted ablation studies on our proposed spatial attention module and multi-scale attention module. 

==> tables/coco20i.tex <==

\begin{table}[ht]
\caption{4-fold split on COCO-20^{i}.}
\resizebox{.49\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{COCO-20^{0}} & \multicolumn{2}{c|}{COCO-20^{1}} & \multicolumn{2}{c|}{COCO-20^{2}} & \multicolumn{2}{c|}{COCO-20^{3}} \\ \hline \hline
1         & Person            & 2         & Bicycle          & 3         & Car              & 4         & Motorcycle       \\ \hline
5         & Airplane          & 6         & Bus              & 7         & Train            & 8         & Truck            \\ \hline
9         & Boat              & 10        & T.light          & 11        & Fire H.          & 12        & Stop             \\ \hline
13        & Park meter        & 14        & Bench            & 15        & Bird             & 16        & Cat              \\ \hline
17        & Dog               & 18        & Horse            & 19        & Sheep            & 20        & Cow              \\ \hline
21        & Elephant          & 22        & Bear             & 23        & Zebra            & 24        & Giraffe          \\ \hline
25        & Backpack          & 26        & Umbrella         & 27        & Handbag          & 28        & Tie              \\ \hline
29        & Suitcase          & 30        & Frisbee          & 31        & Skis             & 32        & Snowboard        \\ \hline
33        & Sports ball       & 34        & Kite             & 35        & B.bat            & 36        & B. glove         \\ \hline
37        & Skateboard        & 38        & Surfboard        & 39        & T. racket        & 40        & Bottle           \\ \hline
41        & W. glass          & 42        & Cup              & 43        & Fork             & 44        & Knife            \\ \hline
45        & Spoon             & 46        & Bowl             & 47        & Banana           & 48        & Apple            \\ \hline
49        & Sandwich          & 50        & Orange           & 51        & Broccoli         & 52        & Carrot           \\ \hline
53        & Hot dog           & 54        & Pizza            & 55        & Donut            & 56        & Cake             \\ \hline
57        & Chair             & 58        & Couch            & 59        & P. plant         & 60        & Bed              \\ \hline
61        & D. table          & 62        & Toilet           & 63        & TV               & 64        & Laptop           \\ \hline
65        & Mouse             & 66        & Remote           & 67        & Keyboard         & 68        & Cellphone        \\ \hline
69        & Microwave         & 70        & Oven             & 71        & Toaster          & 72        & Sink             \\ \hline
73        & Fridge            & 74        & Book             & 75        & Clock            & 76        & Vase             \\ \hline
77        & Scissors          & 78        & Teddy            & 79        & Hairdrier        & 80        & Toothbrush       \\ \hline
\end{tabular}
}
\caption{
COCO-$20^i$ category splits. For the i-th fold, the images of the 20 classes of the i-th split are used for evaluation, and the other images of the other splits are used for training.
}
\label{tablecoco20i}
\end{table}

==> tables/pascal5i.tex <==
\begin{table}[ht]
\centering
\resizebox{.45\textwidth}{!}{%
\begin{tabular}{|c|c|} %p{1cm} 
\hline
Dataset & Unseen classes \\ \hline\hline
PASCAL-$5^{0}$ & aeroplane, bicycle, bird, boat, bottle   \\ \hline
PASCAL-$5^{1}$ & bus, car, cat, chair, cow   \\\hline
PASCAL-$5^{2}$ & diningtable, dog, horse, motorbike, person   \\\hline
PASCAL-$5^{3}$ & potted plant, sheep, sofa, train, tv/monitor \\\hline
\end{tabular}}
\caption{Unseen classes for a four split cross-validation test on PASCAL-$5^{i}$ dataset}
\label{table:pascal}
\end{table}
